Communication-aware Multi-agent Systems Control Based on $k$-hop Distributed Observers

We propose a distributed control strategy to allow the control of a multi-agent system requiring k-hop interactions based on the design of distributed state and input observers. In particular, we design for each agent a finite time convergent state and input observer that exploits only the communication with the 1-hop neighbors to reconstruct the information regarding those agents at a 2-hop distance or more. We then demonstrate that if the k-hop based control strategy is set-Input to State Stable with respect to the set describing the goal, then the observer information can be adopted to achieve the team objective with stability guarantees.

==> content/Problem_formulation.tex <==
 

==> content/notation.tex <==
\textbf{Notation}: We denote by $\mathbb{R}$ and $\mathbb R_{\ge 0}$ the set of real and non-negative real numbers, respectively. Let the cardinality of a set $S$ be represented as $|S|$, $\mathbb{R}^n$ be an $n$-dimensional Euclidean space and $\mathbb{R}^{n \times m}$ be a space of real matrices with $n$ rows and $m$ columns. Denote by $I_n$ the identity matrix of size $n$ and by $1_n = [1, \dots,1]^\top$ the vector of ones of size $n$. Given a matrix $B \in \mathbb{R}^{n\times n}$, we represent with $\lambda_i(B)$, $\lambda_{\text{min}}(B)$ and $\lambda_{\text{max}}(B)$ respectively the $i$-th, minimum and maximum eigenvalues of $B$. Additionally, given a positive definite matrix $B=B^\top \succ 0$ and a vector $x \in \mathbb{R}$, $\norm{x}_B= \sqrt{x^\top B x}$, with the convention $\norm{x}=\norm{x}_I$.
Let $\text{diag}(a_1, \dots, a_n)$ be the diagonal matrix with diagonal elements  $a_1, . . . , a_n$ and let $\otimes$ be the Kronecker product. 
We denote by $\text{sign}(x)$ the non-smooth function defined as:
\begin{equation}
    \sign(x) = \begin{cases}
        1 \hspace{1cm} \text{if } x \geq 0  \\
        -1 \hspace{0.75cm} \text{if } x < 0 
    \end{cases}.
\end{equation}
Given the presence of the $\sign(\cdot)$ function in the observers' dynamic, the non-smooth theory is required to study their convergence. For this purpose, as in \cite[(1.2a)]{4048815}, we denote the set value map of a measurable, locally bounded function $f(y): \mathbb{R}^m \rightarrow  \mathbb{R}^m$ as:
\begin{equation}
    K[f](y) := \bigcap_{\delta>0}\bigcap_{\mu\{M\}=0}\overline{\text{co}}\{ f(\mathcal{B}(y,\delta)/M)\},
\end{equation}
where $\mathcal{B}(y,\delta)$ denotes the ball of radius $\delta$ centered at $y$, $\cap_{\mu\{M\}=0}$ the intersection over all sets $M$ of Lebesgue measure zero, $\mathcal{B}(y,\delta)/M$ the set difference between $\mathcal{B}(y,\delta)$ and $M$ and $\overline{\text{co}}$ the convex combination.
Moreover, we further define:
\begin{equation}
    \norm{K[f]}= \sup_{z \in R(K[f])} \norm{z},
\end{equation}
where $R(K[f]) =  \bigcup_{y \in \mathbb{R}^m} K[f](y)$.
